A complete classification of 2d symmetry protected states with symmetric entanglers

We consider symmetry protected topological states of 2d quantum spin systems, with a finite symmetry group $G$. It has been conjectured that such states are classified by the cohomology group $H^3(G,U(1))$, but the completeness of this classfication is an open problem. We restrict ourselves to symmetry protected topological states that can be prepared from a product state by a symmetric entangler. For this class of states, we prove that the classification by $H^3(G,U(1))$ is complete.

==> myPackage.tex <==
\usepackage{graphicx,xcolor,textpos}

\graphicspath{{./img/}{./Images/}}

\usepackage{}
\usepackage{helvet}
\usepackage[english]{babel}
\usepackage[normalem]{ulem}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{thmtools,thm-restate}
\usepackage{bbm}
\usepackage{amssymb}
\usepackage{hyperref}
\usepackage{relsize}
\usepackage[left=1in, right=1in, top=1in, bottom=1in]{geometry}
\usepackage{physics}
\usepackage[shortlabels]{enumitem}
\usepackage{mathtools}
\usepackage{changepage}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{verbatim}
\usepackage{url}
\usepackage{standalone}
\usepackage{tikz}
\usetikzlibrary{calc,patterns,angles,quotes}
\usepackage{dsfont}
\usepackage{mathrsfs}
\usepackage[affil-it]{authblk}
\usepackage{titlesec}
\usepackage[countmax]{subfloat}

\makeatletter
\newcommand\Label[1]{&\refstepcounter{equation}(\theequation)\ltx@label{#1}&}
\makeatother

\newcommand{\stkout}[1]{\ifmmode\text{\sout{\ensuremath{#1}}}\else\sout{#1}\fi}
\newcommand{\IAC}{\textrm{IAC}}
\newcommand{\cone}{\textrm{Cone}}
\renewcommand{\d}{\text{d}}
\renewcommand{\O}{\mathcal{O}}
\newcommand{\e}{\mathlarger{e}}
\newcommand{\defeq}{\vcentcolon=}
\newcommand{\Hsplit}{{H_{\text{split}}}}
\newcommand{\HsplitTilde}{{\tilde{H}_{\text{split}}}}
\newcommand{\phiTilde}{\tilde{\phi}}
\DeclareMathOperator{\reg}{reg}
\DeclareMathOperator{\C}{\mathbb{C}}
\DeclareMathOperator{\End}{End}
\DeclareMathOperator{\Hilb}{\mathcal{H}}
\DeclareMathOperator{\rreg}{\rho_{\reg}}
\DeclareMathOperator{\swap}{swap}
\DeclareMathOperator{\range}{range}
\newcommand{\trreg}[1]{\rho^{#1}_{\reg}}
\newcommand{\id}{\mathrm{id}}

\newcommand{\Span}{\mathrm{span}}


\let\originalleft\left
\let\originalright\right
\renewcommand{\left}{\mathopen{}\mathclose\bgroup\originalleft}
\renewcommand{\right}{\aftergroup\egroup\originalright}
\let\al\alpha

\newcommand{\UU}{\mathcal U}
\newcommand{\KK}{\mathcal K}
\newcommand{\BB}{\mathcal B}
\newcommand{\PP}{\mathcal P}
\newcommand{\HH}{\mathcal H}
\newcommand{\ZZ}{\mathbb Z}
\newcommand{\CC}{\mathbb C}
\newcommand{\TT}{\mathbb T}
\renewcommand{\AA}{\mathcal A}
\newcommand{\A}{\mathcal A}
\newcommand{\LL}{\mathcal L}
\newcommand{\RR}{\mathbb R}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\1}{\mathbbm{1}}
\newcommand{\alg}[1]{\mathcal{A}_{\ZZ^{#1}}}


\DeclareMathOperator{\Fusion}{\Phi}
\DeclareMathOperator{\Crossing}{\Psi}

\DeclareMathOperator{\supp}{\mathrm{supp}}

\DeclareMathOperator{\ano}{\Omega}
\DeclareMathOperator{\Obstruction}{\Lambda}

\DeclareMathOperator{\proj}{\mathrm{proj}}

\DeclareMathOperator{\rev}{\mathrm{rev}}

\newcommand{\sfA}{\mathsf{A}}
\newcommand{\sfB}{\mathsf{B}}
\newcommand{\sfC}{\mathsf{C}}
\providecommand{\edit}[1]{#1}
\providecommand{\editcolor}{}
\newcommand{\sfU}{\edit{\mathsf{U}}}
\newcommand{\sfV}{\edit{\mathsf{V}}}
\newcommand{\sfD}{\edit{\mathsf{D}}}
\newcommand{\sfTheta}{\mathsf{\Theta}}



\newcommand{\ie}{i.e.\;}


\newcommand{\caA}{\mathcal{A}}
\newcommand{\caB}{\mathcal{B}}
\newcommand{\caC}{\mathcal{C}}
\newcommand{\caD}{\mathcal{D}}
\newcommand{\caE}{\mathcal{E}}
\newcommand{\caL}{\mathcal{L}}
\newcommand{\caM}{\mathcal{M}}
\newcommand{\caN}{\mathcal{N}}
\newcommand{\caR}{\mathcal{R}}
\newcommand{\caS}{\mathcal{S}}
\newcommand{\caP}{\mathcal{P}}
\newcommand{\caU}{\mathcal{U}}
\newcommand{\bbZ}{\mathbb{Z}}
\newcommand{\bbC}{\mathbb{C}}
\newcommand{\bbN}{\mathbb{N}}
\newcommand{\bbR}{\mathbb{R}}
\newcommand{\caF}{\mathcal{F}}
\newcommand{\bulk}{\mathrm{int}}
\newcommand{\wA}{\widetilde\AA}
\newcommand\restr[2]{\ensuremath{\left.#1\right|_{#2}}}
\newcommand{\caI}{\mathcal{I}}
\newcommand{\ind}{\mathrm{ind}}

\newcommand{\diam}{\mathrm{diam}}


\renewcommand{\AA}{\mathcal A}

\renewcommand{\RR}{\mathbb R}

\newcommand{\caal}{\caA_{\textrm{al}}}
\newcommand{\stack}{\tilde \otimes}
\newcommand{\charge}{^{(c)}}
\newcommand{\chargep}{^{(c')}}
\newcommand{\spacing}{\vspace{.5cm}}


\DeclareMathOperator{\CZ}{CZ}
\DeclareMathOperator{\I}{\mathbf{1}}
\DeclareMathOperator{\Z}{\mathbb{Z}}

\newcommand{\Ad}[1]{\textrm{Ad}\left(#1\right)}
\newcommand{\Aut}[1]{\textrm{Aut}\left(#1\right)}
\newcommand{\QAut}[1]{\textrm{QAut}_1\left(#1\right)}
\newcommand{\Herm}[1]{\textrm{Herm}\left(#1\right)}

\newcommand{\qe}{\underset{\text{q.e.}}{\sim}}
\newcommand{\ue}{\underset{\text{u.e.}}{\sim}}

\newcommand{\Mod}[1]{\mathrm{mod} #1}

\DeclareMathOperator*{\slim}{s-lim}


\newtheoremstyle{exampstyle}
{15pt} % Space above
{15pt} % Space below
{\itshape} % Body font
{} % Indent amount
{\bfseries} % Theorem head font
{.} % Punctuation after theorem head
{.5em} % Space after theorem head
{} % Theorem head spec (can be left empty, meaning `normal')

\theoremstyle{exampstyle}

%\theoremstyle{definition}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{definition}[theorem]{Definition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{example}[theorem]{Example}
\newtheorem{proposition}[theorem]{Proposition}


\newenvironment{proofof}[1][]{\emph{Proof of #1 : }}{\hfill$\qedsymbol$\vskip.5cm}



\DeclareMathOperator{\Ker}{\mathrm{Ker}}
\DeclareMathOperator{\Ran}{\mathrm{Ran}}
\DeclareMathOperator{\dist}{\mathrm{dist}}
\DeclareMathOperator{\flow}{\mathrm{flow}}
\DeclareMathOperator{\QCA}{\mathsf{QCA}}
\DeclareMathOperator{\Sym}{\mathsf{Sym}}
\DeclareMathOperator{\sEnt}{\mathsf{sEnt}}
\DeclareMathOperator{\SE}{\mathsf{SE}}
\DeclareMathOperator{\sSPT}{\mathsf{SPT}^{\mathsf{SE}}}
\DeclareMathOperator{\sSta}{\mathcal{S}}


\newcommand{\J}{y}
\newcommand{\Left}[1]{L_{#1}}
\newcommand{\interior}{\mathrm{int}}
\newcommand{\emb}[1]{\xhookrightarrow{#1}}
\usepackage{tikz-cd}
\usetikzlibrary{positioning,fit,calc}
